Are Neuromorphic Architectures Inherently Privacy-preserving? An Exploratory Study

While machine learning (ML) models are becoming mainstream, especially in sensitive application areas, the risk of data leakage has become a growing concern. Attacks like membership inference (MIA) have shown that trained models can reveal sensitive data, jeopardizing confidentiality. While traditional Artificial Neural Networks (ANNs) dominate ML applications, neuromorphic architectures, specifically Spiking Neural Networks (SNNs), are emerging as promising alternatives due to their low power consumption and event-driven processing, akin to biological neurons. Privacy in ANNs is well-studied; however, little work has explored the privacy-preserving properties of SNNs. This paper examines whether SNNs inherently offer better privacy. Using MIAs, we assess the privacy resilience of SNNs versus ANNs across diverse datasets. We analyze the impact of learning algorithms (surrogate gradient and evolutionary), frameworks (snnTorch, TENNLab, LAVA), and parameters on SNN privacy. Our findings show that SNNs consistently outperform ANNs in privacy preservation, with evolutionary algorithms offering additional resilience. For instance, on CIFAR-10, SNNs achieve an AUC of 0.59, significantly lower than ANNs' 0.82, and on CIFAR-100, SNNs maintain an AUC of 0.58 compared to ANNs' 0.88. Additionally, we explore the privacy-utility trade-off with Differentially Private Stochastic Gradient Descent (DPSGD), finding that SNNs sustain less accuracy loss than ANNs under similar privacy constraints.

==> Sections/DPSGD.tex <==

\titleformat{\section}
  {\normalfont\Large\bfseries}{\thesection}{1em}{}
\titleformat{\subsection}
  {\normalfont\large\bfseries}{\thesubsection}{1em}{}

\titlespacing*{\section}
  {0pt}{0.5ex plus 1ex minus .2ex}{0.3ex plus .2ex}
\titlespacing*{\subsection}
  {0pt}{0.5ex plus 1ex minus .2ex}{0.3ex plus .2ex}
\subsection{\textbf{DPSGD Setup}}
We implement DPSGD shown in Figure~\ref{fig:dpsgd} using Opacus framework\cite{yousefpour2021opacus}. 

To investigate the privacy-utility tradeoff, we define the same target privacy budget ($\varepsilon$), while fixing the privacy compromise $\delta=1e-5$ and evaluate the utility of the SNN architectures comparatively with their ANN counterparts. 

% Table~\ref{tab:dpsgd_params} details the DPSGD parameters required for balancing privacy and performance during neural network training. 

% The learning rate, $\eta_t$ determines the magnitude of weight adjustments during gradient descent, while the noise multiplier, $\sigma$ ~\cite{shockley1938theory} controls the amount of noise added to the gradients to maintain privacy. The privacy parameter \(\delta\) represents the acceptable probability of privacy compromise, and the maximum per-sample gradient norm (\textit{C}) limits each sample's influence on the output by clipping gradients. 

% \textbf{\begin{table}[htp]
% \centering
% \caption{DP-SGD Parameters}
% \label{tab:dpsgd_params}
% \begin{tabular}{lc}
% \toprule
% \textbf{Parameter} & \textbf{Value} \\
% \midrule
% Learning rate ($\eta$) & $0.1$ \\
% Noise multiplier ($\sigma$) & $1$ \\
% Privacy parameter ($\delta$) & $1e-5$ \\
% Gradient norm ($C$) & $1.0$ \\
% \bottomrule
% \end{tabular}
% \end{table}
% }







==> Sections/Experimental_setup.tex <==
\section{Experimental Setup}
\input{Sections/Model_arch}
\input{Sections/MIA}
\input{Sections/DPSGD}




==> Sections/MIA.tex <==






\subsection{\textbf{Attack Setup:}}

In this research, we implemented MIA using a two-model approach as illustrated in Figure~\ref{fig:mia_24}. Our experimental setup includes a `target' model, trained on the entire dataset, and a `shadow' model that simulates the target's functionality, trained on 80\% of the same data. Both models share an identical architectural framework.

We evaluate both models by querying them with their respective training sets and distinct test sets. We label the responses as `IN' if the data was in the model's training set and `OUT' otherwise. To prevent the classifier's bias towards the more frequent classes, we balance the distribution of `IN' and `OUT' labels by downsampling the predominant class. We train a Support Vector Machine (SVM) \cite{joachims1998making} on these labeled predictions from the shadow model, and test it with similar data from the target model. Our assessment focuses on the SVM's ability to accurately classify `IN' and `OUT' data, quantified through the ROC curve \cite{hoo2017roc} and the AUC \cite{bradley1997use} metrics, providing a detailed measure of the model’s susceptibility to MIA.



==> Sections/Methodology.tex <==
\section{Methodology}
Our methodology consists of two main components: an experimental framework and an SNN exploration space as illustrated in Figure~\ref{fig:flow}. The experimental framework is designed to assess the privacy leakage and privacy-utility trade off of both ANN and SNN models, while the SNN exploration space investigates the impact of various SNN architectures and hyperparameters on model performance and privacy
\subsection{\textbf{Experimental Framework}}
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.8\linewidth, height=\linewidth]{Figure/mia_1sm.png}
    % \includegraphics[width=\linewidth]{Figure/mia_1sm.png}
    \caption{Membership Inference Attack(MIA) Framework}
    \label{fig:mia_24}
\end{figure}
\subsubsection{\textbf{Privacy Leak Assessment: }}
\label{subsubsec:resiliency}
In this section, we employ MIA as a tool to assess and compare the privacy-preserving properties of SNNs and ANNs. We train the baseline ANN and SNN models on simpler datasets (MNIST~\cite{lecun2010mnist}, F-MNIST~\cite{xiao2017fashion}, Iris~\cite{omelina2021survey}, Breast Cancer~\cite{misc_breast_cancer_14}) and utilize deep architectures on more complex datasets (CIFAR-10~\cite{cifar10}, CIFAR-100~\cite{recht2018cifar}, ImageNet~\cite{deng2009imagenet}) as discussed in Section~\ref{subsec:arch}. To evaluate the models' vulnerability to MIAs, we use  AUC under the ROC curve metric. A higher AUC value indicates a greater susceptibility to MIAs, while a lower AUC value suggests better privacy preservation.
By comparing the AUC values obtained from MIAs on ANN and SNN models across different datasets and architectures, we can assess the relative privacy-preserving capabilities of these two model types. If SNNs consistently demonstrate lower AUC values compared to ANNs, it would suggest that SNNs provide superior privacy protection against MIAs compared to the traditional approach of ANNs.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.9\linewidth]{Figure/dpsgd.png}
    \caption{Differential Privacy via Stochastic Gradient Descent (DPSGD) Algorithm}
    \label{fig:dpsgd}  
\end{figure}
\subsubsection{\textbf{Privacy-Utility Trade off Assessment}}
\label{subsubsec:dpsgd}

We investigate the privacy-utility trade off of the ANN and SNN models by applying DPSGD as a privacy defense mechanism on their training loop. We train these models on MNIST, Fashion-MNIST, Iris, and Breast Cancer datasets, using the Opacus library for integrating differential privacy.
We vary the privacy budget $(\epsilon$) to assess the impact of DPSGD on the privacy-utility trade off. Lower $(\epsilon$) values provides stronger privacy but may reduce model utility, measured by classification accuracy on test sets. We compare the accuracy of ANN and SNN models under different privacy budgets and plot the accuracy against $(\epsilon$) values to visualize the privacy-utility relationship (Figure~\ref{fig:dp_acc}). If SNNs exhibit better performance compared to ANNs when subjected to the same privacy constraints, it indicates that SNNs may provide inherent robustness against the noise introduced by privacy preserving techniques.

\begin{algorithm}[H]
\caption{DPSGD Algorithm}
\label{alg:dpsgd}
\begin{algorithmic}[1]
\State \textbf{Input:} Dataset $\{x_1, \dots, x_N\}$, loss function $\mathcal{L}(\theta) = \frac{1}{N}\sum_{i=1}^N \mathcal{L}(\theta, x_i)$
\State \textbf{Parameters:} Learning rate $\eta$, noise scale $\sigma$, batch size $L$, gradient norm bound $C$
\State Initialize $\theta_0$ randomly
\For{$t = 1$ \textbf{to} $T$}
\State Take a random sample $L_t$ with sampling probability $\frac{L}{N}$
\For{each $i \in L_t$}
\State Compute gradient $g_t(x_i) \leftarrow \nabla_\theta \mathcal{L}(\theta_t, x_i)$
\State Clip gradient $g_t(x_i) \leftarrow \frac{g_t(x_i)}{\max(1, \frac{\|g_t(x_i)\|_2}{C})}$
\EndFor
\State Add noise $\tilde{g}_t \leftarrow \frac{1}{L} \left(\sum_{i \in L_t} g_t(x_i) + \mathcal{N}(0, \sigma^2 C^2 I)\right)$
\State Update parameters $\theta_{t+1} \leftarrow \theta_t - \eta \tilde{g}_t$
\EndFor
\State \textbf{Output:} Return $\theta_T$ and compute privacy cost $(\epsilon, \delta)$
\end{algorithmic}
\end{algorithm}

The DPSGD algorithm ~\ref{alg:dpsgd} starts by selecting a minibatch $L_t$ uniformly from the set of indices $\{1, \dots, N\}$ with size $L$. For each data point $x_i$ in the minibatch, the gradient of the loss function $\mathcal{L}(\theta_t, x_i)$ with respect to the parameters $\theta_t$ is computed as $g_t(x_i)$. These gradients are then clipped using an $L2$ norm operation, $\hat{g}_t(x_i) = g_t(x_i) / \max(1, \|g_t(x_i)\|_2 / C)$. Gaussian noise $\mathcal{N}(0, \sigma^2 C^2 I)$ is added to the average of the clipped gradients, with $\sigma$ being the noise scale, to ensure differential privacy. The noisy gradient $\tilde{g}_t$ is used to update the model parameters: $\theta_{t+1} = \theta_t - \eta_t \tilde{g}_t$.
\subsection{\textbf{SNN Exploration Space}}
\label{subsec:exploration}

In the SNN exploration space as shown in Figure~\ref{fig:flow}, we investigate two major learning algorithms: surrogate gradient-based learning ~\cite{neftci2019surrogate} and evolutionary learning~\cite{schuman2020evolutionary}. 
\subsubsection{\textbf{Surrogate Gradient based Learning:}}

Surrogate gradient-based learning algorithms are used to train Spiking Neural Networks (SNNs) by approximating the non-differentiable spiking function with a differentiable surrogate. This allows the application of gradient-based optimization techniques, such as backpropagation, to SNNs. By replacing the true gradient of the spike function with a smooth, differentiable approximation, these algorithms enable the effective training of SNNs. In our experiments, we employ the Arc-tangent ~\cite{1628884} surrogate gradient algorithm through the snnTorch ~\cite{snn} framework and the  Spike-Timing-Dependent Plasticity (STDP) ~\cite{caporale2008spike} learning rule using the LAVA~\cite{lava2023}  framework by Intel. 




\noindent{\textbf{snnTorch Framework:}}

snnTorch  is a deep learning framework specifically designed for SNNs built on PyTorch. For our experiments, we utilized the arc tangent learning algorithm within the framework. This algorithm approximates the non-differentiable spiking function with an arc tangent function. This framework was applied to MNIST, F-MNIST, Iris and Breast Cancer datasets to evaluate the resilience of SNNs against MIA.

In SNNs, encoding refers to the process of converting input data into spike trains that the network can process and it determines how input signals are represented as spikes, which regulates performance and behavior of the SNNs.

We explore the impact of different encoding schemes on privacy preserving properties of SNNs. The three encoding schemes ~\cite{snntorch} we investigated on snnTorch are:

\begin{itemize}
    \item \textbf{Rate Encoding:} Transforms input features into spikes by representing each feature as a probability of spike occurrence at each time step, with the neuron's firing rate directly tied to the intensity of the input signal. For our experiments, we set number of steps to 10.
    \item \textbf{Latency Encoding:} Encodes information based on the timing of spikes, where inputs with higher values result in earlier spikes, effectively using the temporal dimension to convey input magnitude. We used time step of 10 and set the RC constant,  \textit{Tau} to 5, and Threshold to 0.1 for our experiments.
    \item \textbf{Delta Encoding:} Event-driven and produces spikes in response to changes in input features over time, making it adept at capturing dynamic variations in data. In our experiments, we set the threshold to 0.1.
\end{itemize}



\noindent{\textbf{LAVA Framework:}}

LAVA is an innovative open-source software framework designed for neuromorphic computing ~\cite{roy2019towards}. It provides a versatile and flexible environment for developing, simulating, and deploying neuromorphic applications. By abstracting hardware details through a process-based model, LAVA enables the creation of scalable and modular systems that can operate asynchronously across various neuromorphic and conventional hardware platforms. The framework supports rapid prototyping and detailed optimization, making it accessible to both researchers and developers interested in leveraging the unique capabilities of neuromorphic technologies. LAVA aligns particularly well with Intel's Loihi chip ~\cite{davies2018loihi}, a specialized neuromorphic processor. LAVA provides a seamless interface for developing applications that can efficiently run on Loihi. The LAVA framework also supports Spike-Timing-Dependent Plasticity (STDP), a biological learning rule that adjusts synaptic strengths based on the precise timing of spikes. This mechanism allows SNNs to learn temporal patterns and adapt to dynamic inputs. In our experiment, we used framework to evaluate the model's resilience against privacy attack (MIA).

\subsubsection{\textbf{Evolutionary Learning Algorithm:}}

Evolutionary algorithms, such as the Evolutionary Optimization for Neuromorphic Systems (EONS) ~\cite{schuman2020evolutionary}, are capable of enabling the rapid prototyping of SNN applications. These applications can be adapted to hardware constraints and various learning scenarios, including classification ~\cite{schuman2020automated, schuman2022opportunities} and control tasks~\cite{patton2021neuromorphic, schuman2022evolutionary}. EONS, implemented within the TENNLab framework, facilitates the co-design process between neuromorphic hardware and software, helping developers optimize neural network structures within the constraints of neuromorphic hardware. EONS interacts seamlessly with a wide variety of devices ~\cite{schuman2020evolutionary}, architectures ~\cite{10.1145/3381755.3381758}, and application ~\cite{8573122} without necessitating any modifications to its underlying algorithm. This approach, implemented within the TENNLab framework, utilizes an evolutionary algorithm to optimize neuromorphic network structure and weights. This process begins with generating a population of potential network solutions, which can be either randomly created or seeded with pre-existing networks ~\cite{schuman2020evolutionary}. The EONS process then evaluates these networks for fitness based on user-defined criteria and uses common genetic algorithm selection techniques such as tournament or fitness score to choose the most promising networks for reproduction. During reproduction, selected parent networks undergo crossover to swap segments of their structure and merging, which combines their entire structures into a single offspring. Mutation operations introduce random modifications to a network's nodes and edges, facilitating diversity and adaptation in the population. These operations are performed on a generalized network representation consisting of nodes and edges, allowing flexibility and adaptability across different hardware implementations. The entire EONS cycle, designed to optimize network parameters and structure efficiently, repeats until achieving desired performance metrics.

In our experiments we depict the impact of different EONs parameters, encoders and neuro processors inside the framework on the vulnerability of the SNN model against MIA on Iris and Breast Cancer dataset.

\begin{itemize}
\item \textbf{Population Size:}
In the EONS approach, population consists of potential solutions that form the genetic pool for evolution. This initial population can be randomly generated or seeded with pre-existing solutions. Each network is evaluated, and the best-performing networks are selected for reproduction. In our experiments, we vary the population size over 50, 100, 200 and 400 to understand its impact on resilience against MIAs.


\item \textbf{Mutation Rate:}
The mutation rate in the EONS approach specifies the frequency at which random changes are introduced to the solutions. These mutations are essential for exploring new solution spaces and preventing the population from stagnating in local optima. Mutations can be structural, such as adding or deleting nodes and edges, or they can involve changes to parameters like thresholds or weights. In our experiments, we vary the mutation rate over 0.1, 0.5 and 0.9 to study its effects on the inherent privacy preservation in SNNs. 
 
\item \textbf{Crossover Rate:}
The crossover rate determines how often parts of two solutions are recombined to create new solutions, enhancing genetic diversity. In EONS, the algorithm uses a node-edge recombination method, where it mixes components from parent networks to form child networks. By varying the crossover rate, the algorithm maintains a diverse genetic pool which is essential for exploring the solution space and identifying high-performing network configurations. By varying the crossover rate over 0.1, 0.5 and 0.9, we aim to explore its impact on the resilience of SNNs against MIAs. 

\item \textbf{Neuroprocessors:}
We explore 3 neuroprocessors available in the TENNLab framework: 

\begin{itemize}
\item \textbf{RISP} ~\cite{plank2022case}: A lightweight neuro processor employing an integrate-and-fire model with discrete time steps for accumulating and evaluating action potentials, suitable for networks with integer synaptic delays.
\item \textbf{Caspian} ~\cite{kulkarni2021training}: Provides a high-level API and a fast spiking simulator integrated with FPGA ~\cite{kuon2008fpga} architecture, enhancing development and deployment of neuromorphic solutions in size, weight, and power-constrained environments.
\item \textbf{RAVENS} ~\cite{foshie2023functional}: A versatile neuroprocessor from TENNLab with multiple implementations including software simulation, microcontroller, FPGA, ASIC~\cite{good2008asic}, and Memristive ASIC ~\cite{weiss2022hardware}(mRAVENS), catering to a wide range of computational needs in neuromorphic systems.
\end{itemize}

\item \textbf{Encoding Techniques:}
\begin{itemize}
\item \textbf{Flip Flop Technique}: It assigns inverted percentage values in even-numbered bins, ensuring smoother transitions and preserving information about minimum values. It is effective in applications like proximity sensing in LIDAR systems ~\cite{plank2019tennlab}.
\item \textbf{Triangle Technique}: It smooths input space by overlapping bins where values rise to 100\% at bin boundaries and then fall, facilitating a more gradual representation of input data. This is useful in refined control applications.
\end{itemize}
\end{itemize}

==> Sections/Model_arch.tex <==
\subsection{\textbf{Model Architecture:}}
\label{subsec:arch}

The baseline ANN model architecture in PyTorch ~\cite{ketkar2021introduction} consists of a flexible input layer adjusted for different datasets such as MNIST~\cite{lecun2010mnist} and Fashion-MNIST~\cite{xiao2017fashion} with a size of 28x28, Iris~\cite{omelina2021survey} with a size of 4, and Breast Cancer~\cite{misc_breast_cancer_14} with a size of 30. The network consists of a hidden layer containing 1000 neurons. The Rectified Linear Unit (ReLU) \cite{li2017convergence, nair2010rectified} serves as the activation function in both the hidden and output layers, along with an Adam optimizer \cite{kingma2014adam} with a learning rate of 0.001. The specific requirements of the dataset being processed determine the output layer's size, such as 10 units for the MNIST dataset corresponding to its ten digit classes, similar for F-MNIST, 3 for Iris, and 2 for the Breast Cancer dataset. 

The baseline SNN model, similar to the ANN, adapts its input layer to accommodate various dataset sizes, from 28x28 pixels for MNIST and Fashion-MNIST to 4 and 30 features for Iris and Breast Cancer, respectively. It features a 1000-neuron hidden layer and utilizes leaky integrate-and-fire (LIF) neurons~\cite{orhan2012leaky} with a decay factor of 0.95 across a temporal resolution of 25 steps. The optimizer is Adam with a learning rate of 0.001. The output layer configuration in the SNN model is identical to that of the ANN model, adjusted for the specific datasets.

Conversely, for CIFAR-10~\cite{recht2018cifar}, CIFAR-100~\cite{sharma2018analysis}, and ImageNet~\cite{deng2009imagenet}, we employ a Deep Neural Network (DNN) model that adopts a ResNet-18 ~\cite{targ2016resnet} architecture and incorporates adaptive group normalization ~\cite{wu2018group}. Multiple residual blocks, each comprising 3x3 convolutional layers paired with ReLU activation, structure the model. Shortcut connections are implemented to facilitate the preservation of gradient flow throughout deeper layers. For the Deep SNN model, we use SpikingJelly ~\cite{spkjly}, an open-source deep learning framework for Spiking Neural Networks (SNN) based on PyTorch. The model, a spiking version of ResNet, integrates adaptive neuronal functions and dynamic thresholds for memory efficiency and computational precision. It utilizes convolutional layers with 3x3 kernels and group normalization, arranged in blocks that increase channel dimensions while reducing spatial dimensions via strided convolutions and 1x1 bottleneck layers. Input robustness is enhanced by a Poisson generator. A surrogate gradient method approximates the derivative of the non-differentiable spike function for effective learning. The architecture  employs an adaptive average pooling layer that dynamically adjusts to the dimensions of the output from the final convolutional block. This pooling might be configured as a 2x2 or 3x3 grid depending on the output feature map size This optimizes the reduction in spatial dimensions necessary for the fully connected layer, which features 10 output units for CIFAR-10 and 100 units for CIFAR-100 to match each dataset's class count.

\begin{table*}[ht!]
\centering
\caption{Comparison of ANN and SNN Resilience to MIA Across Diverse Datasets}
\label{tab:comparison_ann_snn}
\begin{tabular}{lcccccc}
\toprule
\textbf{Dataset} & \multicolumn{3}{c}{\textbf{ANN}} & \multicolumn{3}{c}{\textbf{SNN}} \\
 & \textbf{Train Acc} & \textbf{Test Acc} & \textbf{Attack AUC} & \textbf{Train Acc} & \textbf{Test Acc} & \textbf{Attack AUC} \\
\midrule
\textbf{MNIST}        & 96.09\% & 97.66\% & \textbf{0.61} & 89.94\% & 94.53\% & \textbf{0.51} \\
\textbf{F-MNIST}      & 93.76\% & 89.69\% & \textbf{0.58} & 88.81\% & 83.37\% & \textbf{0.51} \\
\textbf{Cifar-10}     & 97.89\% & 91.21\% & \textbf{0.70} & 89.98\% & 89.36\% & \textbf{0.58} \\
\textbf{Cifar-100}    & 79.82\% & 70.18\% & \textbf{0.85} & 74.64\% & 67.08\% & \textbf{0.54} \\
\textbf{IRIS}         & 100\%   & 96.67\% & \textbf{0.77} & 97.04\% & 96.67\% & \textbf{0.57} \\
\textbf{Breast Cancer}& 99.54\% & 97.37\% & \textbf{0.65} & 99.62\% & 96.98\% & \textbf{0.55} \\
\textbf{ImageNet}     & 79.17\% & 71.43\% & \textbf{0.61} & 73.22\% & 61.32\% & \textbf{0.54} \\
\bottomrule
\end{tabular}
\end{table*}



\begin{figure*}[ht!]
  \centering
  % First row
  \begin{subfigure}{0.245\textwidth}
    \includegraphics[width=\textwidth]{Figure/basic_torch/mnist_basic_torch.png}
    \caption{MNIST}
    \label{fig:mnist_basic_torch}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{0.245\textwidth}
    \includegraphics[width=\textwidth]{Figure/basic_torch/fmnist_basic_torch.png}
    \caption{F-MNIST}
    \label{fig:fmnist_basic_torch}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{0.245\textwidth}
    \includegraphics[width=\textwidth]{Figure/basic_torch/cifar10_basic_torch.png}
    \caption{Cifar-10}
    \label{fig:cifar10_basic_torch}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{0.245\textwidth}
    \includegraphics[width=\textwidth]{Figure/basic_torch/cifar100_basic_torch.png}
    \caption{Cifar-100}
    \label{fig:cifar100_basic_torch}
  \end{subfigure}
  \\ % New line
  % Second row without gaps
  \begin{subfigure}{0.245\textwidth}
    \includegraphics[width=\textwidth]{Figure/basic_torch/imagenet_basic_torch.png}
    \caption{ImageNet}
    \label{fig:imagenet_basic_torch}
  \end{subfigure}%
  \begin{subfigure}{0.245\textwidth}
    \includegraphics[width=\textwidth]{Figure/basic_torch/iris_basic_torch.png}
    \caption{Iris}
    \label{fig:iris_basic_torch}
  \end{subfigure}%
  \begin{subfigure}{0.245\textwidth}
    \includegraphics[width=\textwidth]{Figure/basic_torch/bc_basic_torch.png}
    \caption{Breast Cancer}
    \label{fig:bc_basic_torch}
  \end{subfigure}
  \caption{ROC curves comparing the performance of MIA on ANN and SNN across various datasets}
  \label{fig:beval}
\end{figure*}


==> Sections/random.tex <==
We hypothesize that the potential resilience of SNNs against MIAs is based on two key aspects. Firstly, the non-differentiable and discontinuous nature of SNNs may contribute to their robustness against MIAs. In ANNs, smooth and continuous activation functions (e.g., sigmoid or ReLU) enable models to establish strong correlations between the learned parameters and individual data points. Consequently, an attacker can  exploit these correlations to infer the presence of specific data points in the training set. However, in SNNs, the discrete and spike-based communication between neurons introduces discontinuities in model response. This non-differentiability may weaken the correlation between the model and individual data points, making it more challenging for an attacker to discern the membership of a particular data point in the training set. As a result, the risk of data leakage through MIAs could be further mitigated in SNNs compared to ANNs. Secondly, the unique encoding mechanisms employed by SNNs may further enhance their resilience against MIAs. In SNNs, the input data is converted into spike trains before being processed by the network. This encoding process introduces an additional layer of stochasticity and variability to the data representation. The specific timing and pattern of spikes can vary even for similar input samples, making them less distinguishable from one another. This increased stochasticity in the encoded data may obscure the unique characteristics of individual data points, rendering them more indistinguishable to an attacker attempting to infer their membership in the training set. In contrast, ANNs directly process the raw input data, potentially preserving more distinguishable features that can be exploited by MIAs.



The discrete and event-driven nature of SNNs contributes to their potential robustness against Membership Inference Attacks (MIAs). The non-differentiable spiking activity and inherent discontinuities complicate the extraction of relationships between model parameters and individual data entries. Additionally, SNNs employ unique encoding schemes that transform input data into spike trains, introducing variability and randomness into the representation. The precise timing and sequence of spikes can differ for inputs with similar characteristics, thereby reducing the distinguishability of specific data points. These attributes of SNNs can diminish the likelihood of successful inference attacks, as they obfuscate the presence of particular data points in the training set, thereby enhancing privacy preservation.

SNNs operate on discrete binary spikes for information encoding, making them non-differentiable and discontinuous. Because the abrupt, non-linear transitions between spike and no-spike states disrupt smooth gradient flow, it becomes difficult to precisely trace how specific inputs influence network activations and learned weights. This complexity suggests that MIAs may be more difficult to implement in SNNs. Moreover, the encoding schemes in SNNs convert input features into sequences of spikes based on probabilistic timing and varying firing rates. This results in diverse spike patterns even for similar inputs, adding stochasticity to the data representation.This added randomness makes it difficult to identify patterns, thereby hampering the effectiveness of MIAs.Consequently, if SNNs are inherently more resilient to privacy attacks, we expect that under similar privacy constraints enforced by DPSGD, SNNs should exhibit a lower performance degradation compared to ANNs, owing to their  the inherent complexity of their spike-based processing and encoding techniques. 




this research aimed to investigate the privacy-preserving properties of Spiking Neural Networks (SNNs) in comparison to traditional Artificial Neural Networks (ANNs), focusing on their resilience against Membership Inference Attacks (MIAs). We hypothesized that the unique characteristics of SNNs, such as their non-differentiable and discontinuous nature, as well as their stochastic encoding mechanisms, could potentially enhance their resistance to MIAs.
To test this hypothesis, we designed a comprehensive experimental framework that evaluated the performance of SNNs and ANNs across diverse datasets, including MNIST, F-MNIST, Iris, Breast Cancer, CIFAR-10, CIFAR-100, and ImageNet. Our experiments encompassed various learning algorithms (surrogate gradient-based and evolutionary learning) and programming frameworks (snnTorch, TENNLab, and LAVA) to provide a thorough analysis of the factors influencing the inherent privacy-preserving properties of SNNs.
The key findings of our research are as follows:

SNNs consistently demonstrated superior resilience against MIAs compared to ANNs, as evidenced by the lower Area Under the Curve (AUC) values for the Receiver Operating Characteristic (ROC) curves. Notably, SNNs achieved an AUC of 0.58 on CIFAR-10 and 0.54 on CIFAR-100, compared to 0.70 and 0.85 for ANNs, respectively.
Evolutionary learning algorithms proved to be more effective in enhancing the resilience of SNNs against MIAs compared to gradient-based methods. For the Iris and Breast Cancer datasets, evolutionary algorithms maintained a consistent AUC of 0.50 across all parameters, while gradient-based algorithms yielded AUC scores of 0.57 and 0.55, respectively.
The privacy-utility tradeoff analysis revealed that SNNs experienced a lower accuracy drop compared to ANNs when applying the Differentially Private Stochastic Gradient Descent (DPSGD) algorithm. For the F-MNIST dataset, with privacy guarantees ranging from 0.17 to 1.03, SNNs showed an average accuracy drop of 7.78%, which was significantly lower than the 23.71% drop observed in ANNs.

These findings hold significant importance in the field of privacy-preserving machine learning, as they highlight the potential of SNNs as a more secure alternative to ANNs in privacy-sensitive applications. The inherent properties of SNNs, such as their non-differentiable and stochastic nature, contribute to their enhanced resilience against privacy attacks, making them a promising direction for future research and development.
Furthermore, the superior performance of evolutionary learning algorithms in enhancing the privacy-preserving properties of SNNs opens up new avenues for exploration and optimization in the neuromorphic computing domain. The lower accuracy drop experienced by SNNs when applying privacy-preserving techniques like DPSGD also suggests that SNNs may be better suited for scenarios that require a balance between privacy and utility.
In summary, this research provides a comprehensive analysis of the privacy-preserving properties of SNNs and their potential as a more secure alternative to ANNs. The findings contribute to the growing body of knowledge in the field of privacy-preserving machine learning and neuromorphic computing, paving the way for future research and development in these areas.

In this research we investigate the inherent privacy-preserving properties of Spiking Neural Networks (SNNs) in comparison to traditional Artificial Neural Networks (ANNs). We design a comprehensive experimental framework to subject both types of models to privacy attacks, specifically focusing on their resilience against Membership Inference Attacks (MIAs). We consider the unique characteristics of SNNs, such as their non-differentiable and discontinuous nature, as well as their stochastic encoding mechanisms, as potential factors enhancing their resistance to such attacks.

Our experimental framework encompasses various learning algorithms and programming frameworks, providing a thorough analysis of the factors influencing the privacy-preserving properties of SNNs. Our key findings demonstrate that SNNs has a greater ability to withstand MIAs compared to ANNs. Specially, evolutionary learning algorithms have proven to be more effective than gradient-based methods in strengthening the privacy resilience of SNNs. Additionally, our analysis of the privacy-utility tradeoff reveals that SNNs show less performance degradation than ANNs when applying the Differentially Private Stochastic Gradient Descent (DPSGD) algorithm.

These findings highlight the potential of SNNs as a more secure alternative to ANNs in privacy-sensitive applications making them a promising direction for future research and development. 





 






